The impact of inhomogeneous subgrid clumping on cosmic reionization II: modelling stochasticity

Small-scale density fluctuations can significantly affect reionization but are typically modelled quite crudely. Unresolved fluctuations in numerical simulations and analytical calculations are included using a gas clumping factor, typically assumed to be independent of the local environment. In Paper I, we presented an improved, local density-dependent model for the sub-grid gas clumping. Here we extend this using an empirical stochastic model based on the results from high-resolution numerical simulations which fully resolve all relevant fluctuations. Our model reproduces well both the mean density-clumping relation and its scatter. We applied our stochastic model, along with the mean clumping one and the Paper I deterministic model, to create a large-volume realisation of the clumping field, and used these in radiative transfer simulations of cosmic reionization. Our results show that the simplistic mean clumping model delays reionization compared to local density-dependent models, despite producing fewer recombinations overall. This is due to the very different spatial distribution of clumping, resulting in much higher photoionization rates in the latter cases. The mean clumping model produces smaller HII regions throughout most of the reionization, but those percolate faster at late times. It also causes a significant delay in the 21-cm fluctuations peak and yields lower non-Gaussianity and many fewer bright pixels in the PDF distribution. The stochastic density-dependent model shows relatively minor differences from the deterministic one, mostly concentrated around overlap, where it significantly suppresses the 21-cm fluctuations, and at the bright tail of the 21-cm PDFs, where it produces noticeably more bright pixels.

==> body/chap3.tex <==
\section{Clumping Model Effect on Observational Signature} \label{chap:RTresult}

The sub-grid clumping model employed affects the local IGM recombination rates, which is then reflected in the derived observable signatures of reionization. In order to understand and try to quantify the importance of this choice, we perform three RT simulations where we fix the source production efficiencies of ionizing photons but vary the clumping model. At each time step the
precomputed N-body density fields are used to create a realisation of the corresponding gridded clumping factor, as described in \S\ref{sec:ClumpMod}. These clumping grids are then stored and then provided as additional inputs
to the radiative transfer simulations.


In this section we direct our attention to the results of our RT-simulation with the \texttt{C$^2$-RAY} code. In this first paper, we decided to focus on the larger box only, therefore hereafter we present the obtained outputs from the RT simulation of LB-2. In future project we plan to study a series of large boxes with improved models (e.g, time evolving model, baryonic clumping factor). The goal here is to analyse eventual changes in the observational signature of EoR due to the parametrisation choice of the clumping factor approach. It should be noted that a better understanding of these dependencies allow us to have a more realistic prediction of what we should expect from future observational (e.g, SKA).

As we mention in \S\ref{sec:Nbody}, from the N-Body IGM density field we pre-computed the sub-grid clumping factor for the large, low resolute box LB-2. The simulation redshift range spreads from $z=40$ to $6$, for a total of $125$ snapshots. Therefore, the corresponding aperture on the sky spans from $3.6$ to $\rm4.7\,deg$ and frequency range from $26$ to $\rm45\,MHz$. The data resolution evolves from $43.5$ to $\rm56\,''$ in the spatial direction, while frequency varies from $0.08$ to $\rm0.15\,MHz$.

We study the reionization history in $\S$\ref{sec:IonizHistory} such as the volume averaged ionization fraction $x_i$ evolution, the integrated Thompson optical depth and then the Bubble size distribution in $\S$\ref{sec:BubbleSize}. To better understand the change in ionization morphology we describe a side-by-side comparison of box slice shot with zoom $\S$\ref{sec:SliceComparison}. In \S\ref{sec:21cmSign} we analyse the 21cm signal power spectra and the brightness temperature distribution.

% ---------------------------------------------------------------------------------------------------
\subsection{Ionization History}\label{sec:IonizHistory}
Our simulation are meant to reproduce general reionization features as presented in \cite{Iliev2014}. In high density regions LMACH are the first halos to form. In our simulations they make their first appearance at redshift $z=21$, so that for $z\sim12$ every volume element contain at least one ionizing source. At first, a modest number of isolated sources, highly clustered on small scale but homogeneously distributed on large scale, start to ionize their surrounding gas, forming small regions of a few Mpc size. Throughout reionization, these HII bubbles grow and eventually overlaps, at this point the ionization process accelerates due to the keen opacity drops in ionized region and the subsequent contribution of more then one sources to the expansion of ionization fronts in our simulations.
\begin{figure}
	\hskip-7mm\includegraphics[scale=0.22]{plot_xi} \vskip-2mm
	\caption{Left plot, the volume averaged neutral fraction for BHC (solid red), IC (dashed blue) and SC (solid green). Inset shows the volume average ionization fraction. On the right we show the redshift delay caused by the different clumping approach. Observational constrains are the same as in \protect\cite{Dixon2015}, Figure 1. We add two more recent data (light purple circles) inferred by high redshift quasars spectra \protect\citep{Davies2018}.}
	\label{fig:xi} 
\end{figure}
\begin{table}
	\begin{tabular}{ccccccc} \hline
		Model				& $z_{10\%}$& $z_{30\%}$& $z_{50\%}$& $z_{70\%}$& $z_{90\%}$& $z_{reion}$	\\ \hline\hline
		BHC				& $11.918$	& $9.533$	& $8.118$	& $7.221$	& $6.721$	& $6.483$		\\
		IC				& $11.918$	& $9.611$	& $8.340$	& $7.480$	& $6.905$	& $6.583$		\\
		SC 				& $11.918$	& $9.611$	& $8.340$	& $7.480$	& $6.905$	& $6.549$		\\ \hline
		$\Delta z$			& $0$		& $0.078$	& $0.222$	& $0.259$	& $0.184$	& $0.1$			\\
		$\Delta t\,[Myr]$	& $0$		& $5.8$		& $22.9$	& $34.4$	& $28.9$	& $17.2$	\\ \hline
	\end{tabular}
	\caption{The reionization history obtained in our simulations. The first part lists, for each model, the redshift at which the mean volume ionized fraction $\bar{x}_i$ reaches the relevant reionization milestones of $10\%$, $30\%$, $50\%$, $70\%$ and $90\%$ volume of the gas ionized. The last column $z_{reion}$ indicates the end of reionization, when $99\%$ of the gas volume is ionized. The second section lists the redshift difference and the due time delay in $Myr$.}
	\label{tab:Eor_history}
\end{table}
At first in \autoref{fig:xi}, we compare the volume averaged neutral fraction, this gives us the global history of ionization in our simulations. Contrary to what we could expect, a more realistic treatment of the sub-grid inhomogeneity leads to an earlier end of reionization. The former models diverge from BHC model in the redshift range $z \leqslant 12$, so that universe reionization is accelerated with a maximum delay of $\Delta z \simeq0.3$ at $z\simeq7.5$, corresponding to a time delay of approximately $\rm36\,Myr$, when on average $70\%$ of the universe volume is ionized. Additionally, from the definition of the volume averaged recombination rate $\left< \mathcal{R} \right> = \alpha_{\rm HI}\, C_{\rm HII}  \left< n_{\rm HII} \right>^2 V_{cell}$, we can express the (dimensionless) number of recombination per mean hydrogen atom $\left<n_{\rm H}\right>$, Hubble time $t_H$ and volume element $\rm V_{cell}$ to study the affects on recombination in our simulations.

\begin{figure}
	\hspace{-3mm}\includegraphics[scale=0.32]{plotTaue_comparison}\vskip-3mm
	\caption{Reionization integrated electron-scattering. We overplot the \textit{Planck} observational constrain (black dashed line) with its relative $1$-$\sigma$ confidence interval (violet shadow)} \label{fig:tau}
	\vspace{-5mm}
\end{figure}


\begin{equation}\label{eq:dimrec}
\rm\left< N_{rec} \right> 
%= \frac{\left<\mathcal{R}\right>}{t_H(z)\, \left<n_{\rm H}\right> \, V_{cell}} 
= \frac{2}{3}\, \frac{\alpha_{HI}\, \Omega_b\, \rho_{c,0}}{H_0 \Omega^{1/2}_m \,(1+z)^{3/2} \, \mu_H \, m_p} \, C_{\rm HII} \left< x_{\rm HII} \right>^2
%= \frac{2}{3}\, \frac{\alpha_{HI}\, \Omega_b\, \rho_{c,0}}{H(z) \,\, \mu_H \, m_p} \, C_{\rm HII} \left< x_{\rm HII} \right>^2
\end{equation}

\begin{figure*}
	\hskip-5mm\includegraphics[scale=1.13]{plotRec+Ion} \vskip-2mm
	\caption{Evolution of the volume average recombination per mean hydrogen atom and Hubble time throughout reionization (left) and photoionization rate in our simulation (right). The bottom plots show the relative difference compared to BHC. Shadows area of the same colour indicate the relative quantity in under-dense (lower limit) and over-dense (upper limit) regions.}
	\label{fig:rec+phot} 
\end{figure*}
In \autoref{fig:rec+phot} (left image) we show the volume average of this quantity and in the bottom panel the relative difference in percentage to BHC. At lower redshift the overall larger clumping factor in the sub-grid models leads to a higher recombination rate, as we expected from the consistency check in \autoref{fig:mean_comparison}. The discrepancy starts at redshift $\rm z\simeq12$ and increases as structure form, with relative error that fluctuates between $\rm 80-140\%$. In our simulations \autoref{eq:dimrec} depends explicitly on the clumping factor and the ionization fraction $\rm\left< N_{rec} \right> \propto \mathcal{C}_{\rm HII} \left< x_{\rm HII}\right>^2$, since IC and SC show similar volume averaged ionized fraction, when we compare the dimensionless recombination the only diversity is governed by the clumping factor. SC shows an overall higher recombination rate of a few percent $\sim1-5\%$ compared to IC. This is most likely due to the stochastic nature of the realization process, also explaining the broader standard deviation in \autoref{fig:mean_comparison} (shadow areas).\\

In \autoref{fig:rec+phot} (right image) we compare the photoionization rate $\Gamma_i$ computed by the \texttt{C$^2$-Ray code}. As in the previous case, discrepancies between BHC and the two density dependent models arise at the same redshift. In the above-mentioned model the average source ionization intensity decreases drastically, such that overall IC and SC have almost one times and an half more photoionization radiation for redshift between $z=12$ and $7$. As mentioned before, sources are formed inside gravitational collapse structures and reionization is an inside-out process, where high density regions get ionized before low density regions. Accordingly, a partial suppression is applied for LMACHs that resides within ionized regions ($\bar{x}_i>0.1$) \citep{Dixon2015}. Because the former models higher recombination rate, suppression is slowed down allowing LMACHs to last longer in high density regions. This is clear from \autoref{fig:xi_PDF} where we show the distribution of cells ionization at five different reionization milestones $\bar{x}_i=0.1,\,0.3,\,0.5,\,0.7,\,0.9$, approximately corresponding to redshift between $z\simeq 12-6$ (see \autoref{tab:Eor_history}), the vertical line indicate the partial suppression threshold for LMACHs. At stage $\bar{x}_i=0.3$, the former models are the most similar to each other, at this stage BHC is gaining more ionized cells and at the same time it is starting to show a lack of neutral regions compared to IC and SC. At later stages, when the universe becomes highly ionized $\bar{x}_i=0.5$, the dearth of neutral cells is more prominent whereas the peak of highly ionized cells becomes identical overall the models. A faint difference between SC and IC is visible in the last three plots, where slightly more cells remain neutral in SC, although this is probably inconsequential on the reionization history.\\

This first analysis is in contrast with what can be naively deduced from \autoref{fig:mean_comparison}, despite the introduction of sub-grid clumping increases recombination, \autoref{fig:rec+phot} (left), this also leads to an higher photoionization rate in simulations (right). As shown in \autoref{fig:plot500}, inhomogeneity dependent models as IC and SC increase clumping factor with density, in spite of BHC which harshly neglect the inhomogeneous aspect of the problem. This will affect simulation in two main aspects. Since sources reside inside high density regions their radiation is further attenuated before leaving the cell of origin, decreasing the ionization contribution of the IGM. {\sentencetoverify Moreover, the higher clumping factor will increase the neutral lifetime of cells grid that hosts LMACHs, postponing their partial suppression and counter-intuitively allowing them to ionize the universe earlier}. As shown in \autoref{fig:xi_PDF}, the suppression threshold in BHC is already surpassed for $z=8.118$ ($\bar{x}_i=0.5$). Another consequence is that inhomogeneity dependent approach prevent radiation to freely propagate on large scale, shielding high density region from being ionized by multiple fronts.\\

During reionization, free high energy electrons can interact with CMB photons via inverse Compton scattering, suppressing CMB anisotropies on all scales and polarization on large angular sizes in what is known as the \textit{Sunyaev-Zeldovich} (SZ) effect. The contribution from free electron can be quantified by the integrated Thompson scattering optical depth along the line of sight, given by
\begin{equation}\label{eq:tau}
\tau_e(z) = c\,\sigma_T \int^z_{0} \frac{n_e(z')}{(1+z')\,H(z')} dz' 
\end{equation}
where $\sigma_T = 6.65\times 10^{-25} cm^2$ is the Thompson cross section, $c$ the speed of light and $n_e$ is the electron density at a given redshift.\\

Early stage of EoR is dictated by the presence of low mass haloes ($10^8$-$10^9\Msun$), their abundance grows exponentially from redshift $z\sim10$ to $8$ until more massive halos appears and becomes the major contributor to reionization. Hence, $\tau_e$ is a good indicator of LMACHs influence on reionization initial phases. However, as demonstrated by \cite{Ahn2012}, very low mass halos (\textit{minihalos}), that host PopIII stars, could have started ionizing the universe much earlier and therefore have a more significant impact. From the ionized mass fraction $x_m$ we can evaluate the electron density and estimate the electron-scattering optical depth for our simulations. In \autoref{fig:tau} we show the results and plot the volume mean of \autoref{eq:tau}. Here the inhomogeneity dependent model appears slightly optically thicker meaning that the free electron column density is higher and therefore EoR is in a more advance stage with respect to the BHC run. Regardless of this small difference, we compare the models with the $1$-$\sigma$ error interval of the  \cite{PlanckCollaboration2018}, this experiment constrains the upper limit of EoR for a measured integrated optical depth of $\tau_e=0.054^{+0.007}_{-0.008}$, that correspond to an instantaneous reionization for redshift $z_{reion}= 7.68^\pm 0.79$.

% ---------------------------------------------------------------------------------------------------
\subsection{Slice Plot Comparison} \label{sec:SliceComparison}
Although global averaged quantities, \autoref{fig:xi}, \ref{fig:rec+phot} and \ref{fig:tau} give an overall idea of the reionization history, the goal here is to understand how the sub-grid approach affects the diffusion of radiation and subsequently alter the local disposition of the ionized filed. Therefore, in \autoref{fig:slice_comparison} we show box slice of LB-2 and compare simulation snapshots with same globally averaged ionized fraction. From top to bottom row we have $\bar{x}_i=0.3,\,0.5,\,0.7,\,0.9$ (in \autoref{tab:Eor_history} we list the corresponding redshift at which this occurs and its consequent time delay) and from left to right column we have the different models BHC, IC and SC. Red/crimson regions indicate highly ionized cells $x_i>0.9$, in dark blue neutral regions $x_i<0.1$, and in green/aquamarine the transition phase $x_i\approx0.5$. Within each image we embed a zoom-in region, of $85\mpc$ per side, to better appreciate the morphological changes of a randomly selected under-dense neutral clump, as ionized fronts enfold (bluer blob, right column plots).\\

The side-by-side comparison shows remarkable differences between BHC and the two inhomogeneity dependent models. In the first row, snapshots show the imprint of the first sources, this growing HII bubble start independently to ionize their surrounding IGM with mild transition regions that connect neighbour sources. Across the three model no remarkable difference appears on large scale structure, instead an higher degree of ioniziation around sources arises for inhomogeneity dependent model IC and SC (respectively central and right panel).

From the second row, where $50\%$ of the entire gas volume is ionized, we can see nearby growing regions connecting to each other and starting to highly ionize the linking filament. At this point, accordingly to \autoref{fig:xi_PDF}, all cells in BHC have completely surpassed the threshold limit $x_i=0.1$ for the partial suppression of low mass haloes. For IC (middle) and SC (right column) the degree of ionization around sources is visibly more intense compared to BHC, in fact we can distinguish highly ionized cells clustered around the high density peak, whereas under-dense regions are kept fairly neutral. This diversity is due to the sheer recombination rate in inhomogeneity dependent model, shown in \autoref{fig:rec+phot} (left), that effectively reduces the number of photons able to escape the cells of origin and spread into the neighbour grid elements. This is not the case for BHC, to which clumping factor in high density regions is underestimated and ionizing photons are free to percolate and been absorbed elsewhere in the surrounding IGM, therefore interconnecting filament cells between sources clearly appears extended and in a more advanced neutral-ionized transition (blue/aquamarine).
\begin{figure}
	\hskip-3mm\includegraphics[scale=0.27]{plotPDF_xi_sameXi}\vskip-2mm
	\caption{Ionized cell distribution at redshift $z=11.8,\,9.6,\,8.3,\,7.5,\,6.9$, top to bottom, for model BHC (red), IC (blue) and SC (green). Vertical line (black dashed) indicates the ionization threshold, $x_i=0.1$, for partial suppression of LMACHs.}
	\label{fig:xi_PDF}
\end{figure}
At $x_i=0.7$ (third row), ionizing fronts have grown substantially and overlap regions become strongly ionized. A first look suggests similar structure patchiness on large scale, although from the zoom-in we can observe that BHC has a wider and smoother transition between the ionized/neutral phases, whereas IC and SC show a narrower front, allowing more cells that host under-density to stay neutral. When the same transition region dwell across the three model, density dependent model show more irregularity with occasionally one or few cells appearing slightly more ionized then their surrounding.

Differences in clumps morphology are more evident toward the end of EoR. When $90\%$ of the gas volume is ionized (bottom row), HII bubbles have merged together to form one vast interconnected highly ionized region, in such a way that become impossible to distinguish single source any more. At this stage the vast ionized IGM in IC and SC show variations that follow the higher recombination due to density peak fluctuation, this aspect is namely overlook in BHC and therefore the same regions present an uniform filed, highly ionized $\approx 1$. On the other hand there are no striking difference between IC and SC, except for small variations, of a few pixels of size, on the ionized/neutral boundaries. We suspect that this is numeric artefact due to the stochastic nature of SC. We are developing a more complete clumping model, that we will present in future work, to exclude this uncertainty.

\begin{figure*}%0.152]
	\vskip-3mm\makebox[\linewidth][c]{\includegraphics[scale=0.6]{xi_comparison_for_paper_large}}\vskip-2mm
	\caption{Box slice comparison of LB-2 ionization fraction for different clumping approach. In red/crimson highly ionized regions $x_i>0.9$, in green/aquamarine transition $x_i\approx0.5$ and in dark blue neutral regions $x_i<0.1$. The zoom-in covers an area of $85\mpc$ per side and each pixel represent a volume element of $2.381\mpc$ per side. We compare slices at same global average ionization fraction, from top to bottom row we have $\bar{x}_i=0.3,\,0.5,\,0.7,\,0.9$ (see \autoref{tab:Eor_history} for corresponding redshift). From left to right column respectively the model BHC, IC and SC.}
	\label{fig:slice_comparison} 
\end{figure*}



% ---------------------------------------------------------------------------------------------------
\subsection{Bubble Size Distribution} \label{sec:BubbleSize}

\begin{figure*}
	\includegraphics[scale=0.33]{plotBSD_MFP_xi_xth09} \vskip-2mm
	\caption{Ionized bubble size distribution for LB-2. In red the result for BHC, in blue for IC and in green for SC at volume averaged ionized fraction $\bar{x}_i=0.3,\,0.5,\,0.7,\,0.9$. Vertical lines represent the mean radius size $\bar{R} =\int (R\,dN/dR)dR$ for the respective models.}
	\label{fig:bubble}
\end{figure*}
\begin{figure*}
	\includegraphics[scale=0.33]{plotBSD_FOF_xi_xth09} \vskip-3mm
	\caption{Ionized volume size distribution for LB-2. In red the result for BHC, in blue for IC and in green for SC. Distribution represents stages where the volume averaged ionized fraction is $\bar{x}_i=0.3,\,0.5,\,0.7,\,0.9$.}
	\label{fig:volumes}
\end{figure*}


We analyse the normalized distribution of bubble size $R\,dN/dR$ and the volumes size $V^2\,dN/dV$ of ionized region. In the first case we apply the Mean-Free-Path (MFP) method to identifies ionized regions and associate their size to a characteristic radius, by spherical approximation, so to derive the bubble size distribution (BSD) of ionized regions. For the volumes size distribution, we employ a Friends-of-Friends (FOF) algorithm, this method differs from the previous one because it use linkages in data in order to calculate the volume of interconnected ionized regions. In both cases, we apply a threshold value of $x_{th}=0.9$, since we want to highlight differences in distribution of highly ionized regions that develop around sources.

Results in \autoref{fig:bubble} and \autoref{fig:volumes} show typical traits of percolation process, with volume ranges that correspond to what expected from large simulated box \citep{Iliev2014}. We present our results at four different reionization milestones $\bar{x}_i=0.3,\,0.5,\,0.7,\,0.9$, see \autoref{tab:Eor_history} for corresponding redshift. In the case of BSD-MFP, we calculate the mean bubble size by $\bar{R} =\int (R\,dN/dR)\,dR$, represented by vertical lines. The keen-edged cut-off at $2.381\mpc$, for BSD-MFP, and $13.498\mpc^3$ for BSD-FOF is due to the simulation finite resolution.

Initially, for $\bar{x}_i=0.3$ (top left panel, \autoref{fig:bubble}), LB-2 hosts small HII bubbles with radius smaller then $10\mpc$. For inhomogeneity dependent model IC and SC, distributions present more highly ionized regions, indication of a faster radiation propagation around sources, at this early stage the three distribution peaks at the corresponding size of one cell. The same trend is confirmed in \autoref{fig:volumes}, highly ionized bubble are perceivable less and volumes are smaller. In the case of the BHC model, sizes are condensed between $30-700\,\mpc^3$. On the contrary IC and SC volumes distribution scatters from one cell volume $13.498\mpc^3$ up to a few thousand.

At $\bar{x}_i=0.5$ (top right) bubbles size cover a variety of different volume scales, in this particular case BHC and IC share preference for two distinctive type of volume range, a broad flat distribution (plateau) for scales within $V<10^5\mpc^3$, and one large ionized region. The presence of this lone peak, at $10^5 \mpc^3$ for BHC and $10^6 \mpc^3$ for IC, is a characteristic of percolation process \citep{Furlanetto2015}, which indicates that a few small HII bubbles have started to merge together to form a vast interconnected ionized region, named the \textit{percolation cluster}. Nevertheless, IC distribution is shifted toward bigger sizes, such that the limit for the plateau and the percolation cluster are up to one order of magnitude larger. A narrower separation between these two volume range indicates that the merging of ionized region in BHC has just started \citep{Furlanetto2015, Giri2018}, whereas in the case of IC this process is already ongoing. On the other hand, IC and SC distribution show similarity at small scale but they disagree for larger volumes. The former distribution shows a constant and continuous range of scales from large volumes $V\sim10^6\mpc^3$ down to one cell, sign that ionized regions are in principle less interconnected and therefore the presence of one dominant super cluster has not yet occurred.

Once $50\%$ of the universe is ionized the simulations are dominated by two type of population and the neutral lattice is driven by absorption in IGM. At $\bar{x}_i=0.7$ (bottom left) the majority of HII bubble resides at small and moderately large scale $V<10^4\mpc^3$. This is the limit at which isolate ionized volume can independently grows before being absorbed by the much larger percolation cluster, which in all our cases is in the order of approximately $10^8\mpc^3$. At this stage the three models present similar volume distributions, whereas their BSD-MFP varies. BHC distribution is shifted to smaller scale and its mean radius is more then one $\mpc$ away to the other cases, whereas IC and SC almost perfectly overlap and they present a  lightly smaller average in the case of SC model. The difference in the spherical approximation volume is then up to $405\mpc^3$ when compared BHC to SC and $387\mpc^3$ when compared to IC.
\begin{figure}
	\includegraphics[width=\columnwidth]{plotRMS_LC_dTb_B2km.png}\vspace{-4mm}
	\caption{Differential brightness statistic quantities derived from the lightcones data smoothed on the core baseline of SKA1-Low ($\rm B=2\,km$). Plot on top shows the frequency evolution of the signal root mean squared (RMS). Bottom plot shows the skewness and an inset panel show the frequency evolution of the averaged differential brightness in logarithmic scale.}
	\label{fig:dTb_rms_and_mean}
\end{figure}

Toward the end of reionization, at $\bar{x}_i=0.9$ (bottom right), the volume limit for independent regions to grow before merging is further reduced to $V\sim10^3\,\mpc^3$, while the percolation cluster surpass volumes of $10^8\mpc^3$ in all the three cases. In \autoref{fig:bubble}, the sizes distribution in the BHC model has surpassed the other two, with average radius of $54.84\mpc$. IC and SC show again similar distribution but with an increasing, although irrelevant, difference in the mean radius. Volume distribution in \autoref{fig:volumes} present a similar situation, the only difference between IC and SC consists in the value of the volume merging limit, with a difference up to $1\mpc^3$.

% ---------------------------------------------------------------------------------------------------

\begin{figure*}
	\includegraphics[scale=0.52]{plotLightcone_B2km_dTb}\vspace{-5mm}
	\caption{Smoothed differential brightness comparison, the colour map that shows the smoothed differential brightness $\Delta T_b$ intensity as a function of redshifted \textit{21 cm} signal frequency $\nu_{obs}$ and aperture $\Delta \Omega$. The angular smoothing is performed by a Gaussian Kernel with FWHM $\Delta \theta$, on frequency direction is done by a top-hat kernel with same width, we use a baseline of $B=2\,km$ (maximum baseline of the core of SKA1-Low). The figure shows slice through the simulation and a comparison between BHC (top), IC (middle) and SC (bottom).}
	\label{fig:PL_dTb} 
\end{figure*}

\iffalse
\begin{figure}
	\includegraphics[width=\columnwidth]{plotPDF_21cm}
	\caption{differential brightness PDF for $z=12.603,\,10.110,\,9.026,\,8.064,\,7.305$, from top to bottom}
	\label{fig:21cm_PDF}
\end{figure}
\fi


\subsection{21cm Signal Statistics and Power Spectra} \label{sec:21cmSign}
The hyperfine transition of neutral hydrogen can be used as an observable sign during reionization. Its characteristic emission/absorption line has wavelength $\rm\lambda_0=21\,cm$ and corresponding frequency 1.42 GHz. Radio interferometry telescopes measure the intensity of this signal by quantifying the differential brightness temperature $\rm\delta T_b\equiv T_b-T_{CMB}$ signal from the uv-coverage of patches of the sky, given as:
\begin{equation} \label{eq:dTb}
	\rm \delta T_b = 28\,mK (1+\delta)x_{HI} \left(1-\frac{T_{CMB}}{T_S}\right)\left(\frac{\Omega_b h^2}{0.0223}\right)\sqrt{\left(\frac{1+z}{10}\right)\left(\frac{0.24}{\Omega_m}\right)} 
\end{equation}
here $x_{\rm HI}$ is the fraction of neutral hydrogen and $\rm1+\delta = \left<n_{\rm N,IGM}\right>/\bar{n}_{\rm N,IGM}$ is the IGM N-body overdensity. The differential brightness is characterized by the relation between the CMB temperature $\rm T_{CMB}$ and spin temperature $\rm T_S$ (see \citealt{Furlanetto2006} and \citealt{Zaroubi2012} for extended discussion). \autoref{eq:dTb} saturates when the neutral hydrogen decouples from CMB photons and couples with the IGM gas heated by X-ray sources \citep{Ross2019}, so that $\rm T_{S} \gg T_{CMB}$. This is known as the heating saturated approximation where the signal is for the majority observable in emission, $\rm\delta T_b > 0$, true only at low redshift $z<15$. So in our simulation the approximated differential brightness is dependent on the density distribution of the neutral gas and redshift, such that $\rm \delta T_b \propto \sqrt{1+z}\,(1+\delta)\,x_{HI}$.


From the RT and N-body simulation outputs we can evaluate the differential brightness coeval cube at each time step. The cube is then smoothed in the angular direction by a Gaussian Kernel with a FWHM of $\rm\lambda_0\,(1+z)/B$, where $\rm B=2\,km$ corresponds to the maximum baseline of SKA1-Low core. Smoothing on frequency axis is done by a top-hat kernel with same width. 

In \autoref{fig:PL_dTb} we show the smoothed lightcone derived with \autoref{eq:dTb}, for the three different clumping approach, respectively from top to bottom BHC, IC and SC model. This type of data will in principle maps the 21-cm differential brightness evolution at the observed frequency $\rm\nu_{obs}=\nu_0/(1+z)$, where $\rm\nu_0=1.42\,GHz$ is the rest frame frequency when the signal was emitted at redshift $\rm z$. We then express the comoving box length in corresponding angular aperture of $\rm4.65^{\circ}$ at $\rm z=6.583$. 

At early stage, the I-front has not yet efficiently propagate into the IGM. Here high temperatures indicates that the average signal is for the majority in emission $\rm\delta T_b>30\, mK$ and the fluctuations are correlated to the density distribution. Therefore at low frequency $\rm\nu_{obs}\sim70\,MHz$ there is no visible difference between simulations. As radiation escapes the host halo, it gradually suppresses the averaged signal at large scale and it starts to form small isolated transparent regions $\delta T_b=0\,mK$ around sources. \autoref{fig:PL_dTb} shows that this occurs simultaneously, with similar spatial disposition, for the three simulations at frequency higher then 130 MHz ($z\sim10$), but with different intensity of signal suppression. For example the appearances of the first transparent regions, due to lack of neutral hydrogen, at $\nu_{obs}\simeq\rm147\,MHz$ and angular position $\rm3.2^{\circ}$ and $\rm1.1^{\circ}$ shows that ionization around sources are more consistent for the simulation with inhomogeneity dependent clumping. This is the case even at higher frequency $\nu_{obs}>180\,MHz$ ($z<7$), during the final phases of reionization the morphology and size of the \textit{percolation cluster} strongly depends on the clumping model employed by the simulation. BHC model has  large regions of feeble emission $\sim 3$ mK that are extensively linked together. The IC model shows the same morphology but with considerably smaller and more isolated regions of signal. The SC model, in the other hand, shows a conspicuous lack of signal and regions of emission have only of a few Mpc size.

There are significant variation in the statistic of the differential brightness, derived from Lightcones data, shown in \autoref{fig:dTb_rms_and_mean}. The image shows the root mean squared (RMS) on top, the skewness on the bottom and an inset plot that shows the evolution of the mean brightness in logarithmic scale. The low frequency cut-off is chosen for range where differences between models becomes noticeable. The first regions to get ionized are the highest density peak, initially they are smaller then the interferometer resolution, such that their contributions diminish the averaged $\rm\delta T_b$ without increasing fluctuations. At this stage the signal follows the underlying density field and by construction there is no difference amongst the models. The observed frequency of the RMS dip indicates the timing at which HII regions become larger then the interferometry smoothing scale and eventually start to overlap locally. This is the case at frequency larger then $\rm120\,MHz$ ($z\approx11$). For the IC and SC model, the turnover occurs earlier and with a steeper slope than the BHC model, indication that signal fluctuations increase faster and stronger. Moreover the peak value of the RMS fluctuations varies, in the case of IC and SC models the amplitude is $14 \%$ higher, despite having a lower averaged brightness temperature then the homogeneous case, indication of the fact that the signal is sensible on a more physical treatment of the clumping factor. This is the consequence of a lower clumping factor values in under-dense region, consistent with the conclusion in \autoref{sec:IonizHistory}. The faster propagation of I-front, in the vast low density regions, leads to a earlier second peak in the RMS of the two former approaches. In order of appearance at $\rm\nu_{obs}=165\,MHz$ ($\rm z=7.558$) for SC, 169 MHz ($\rm z=7.338$) for IC and slightly later at 176 MHz ($\rm z=7.060$) for BHC, respectively when the average neutral fraction is $\rm \bar{x}_n=0.33$, 0.28 and 0.25. The subsequent decline is the results of reionization reaching its final stage.

The non-Gaussian nature of the 21-cm signal distribution does not allow the power spectrum to fully disclose the Epoch of Reionization proprieties \citep{Mondal2017}. For this reason we decided to analyse a high order statistic quantity such as the skewness, bottom panel in \autoref{fig:dTb_rms_and_mean}. The skewness is going from negative to positive symmetry at $\rm\nu_{obs}\simeq170\,MHz$, when the volume ionized fraction is close to $\rm x_i = 0.6-0.7$ and the RMS fluctuation reaches its maxima. Differences between models are noticeable only later, once the simulation overpass the peak in fluctuations, at frequency larger then 180 MHz. At this point the skewness increase exponentially.

In \autoref{fig:21cmPk} we compare the 21cm power spectra for models BHC, IC and SC at epoch at which the ionization fraction is $\rm x_i=$0.1, 0.3, 0.5, 0.7, 0.9 and at reionization completion $\rm x_i =$0.99. At first, the 21cm signal follows the underlying density distribution of neutral hydrogen and the power spectra is approximatively a power law in all three cases. 
The flattening of the power spectra is an indication of the expanding ionized region, shifting the signal toward larger scales while suppressing small structures. Interestingly, this characteristic appears at the same scale regardless of the clumping model but modest difference in amplitude of signal.
The stochastic relation between local overdensity and clumping factor comes forth predominately at small scale. At k > 1 $\rm Mpc^{-1}$, IC and SC models start to disagree at middle stage with relative error of $\rm5\%$ and increase at later time with $\rm<20\%$. Whereas, at larger scale difference start low at $\rm2\%$ and soar up to $35\%$ only toward reionization end. Compared to BHC the stochastic model has overall more power at all scale size, especially at large scale k < 0.2 $\rm Mpc^{-1}$, where the fractional error is about several hundreds of percentage at $\rm x_i=0.3$. The situation is reversed from $\rm x_i=0.7$, also the relative error at low k is reduced down to $\rm 20\%$, whereas error at large k peaks at $\rm 250\%$ at reionization end $z_{reion}$.

{\workinprogress MICHELE: I have to finish to describe 21cm power spectra}



\begin{figure*}
	\includegraphics[width=\textwidth]{plot_21cmPk}
	%\includegraphics[scale=0.42]{plot_21cmPk_large}
	\caption{The effect of clumping factor on the 21cm power spectra compared at volume ionization fraction $\rm x_i=0.1$, 0.3, 0.5, 0.7, 0.9 and 0.99 for the models under study: BHC (red, solid), IC (blue, dashed) and SC (green, solid).}
	\label{fig:21cmPk} 
\end{figure*}




